Using Staged Tree Models for Health Data: Investigating Invasive Fungal Infections by Aspergillus and Other Filamentous Fungi

Machine learning models are increasingly used in the medical domain to study the association between risk factors and diseases to support practitioners in predicting health outcomes. In this paper, we showcase the use of machine-learned staged tree models for investigating complex asymmetric dependence structures in health data. Staged trees are a specific class of generative, probabilistic graphical models that formally model asymmetric conditional independence and non-regular sample spaces. An investigation of the risk factors in invasive fungal infections demonstrates the insights staged trees provide to support medical decision-making.

==> figures/Tree1.tex <==
\begin{figure}
\centering
\scalebox{0.55}{
\begin{tikzpicture}
\renewcommand{\xx}{2}
\renewcommand{\yy}{1}
\node (v0) at (0*\xx,0*\yy) {\sage{cyan}{0}};
\node (v1) at (1*\xx,-8*\yy) {\sage{black}{1}};
\node (v2) at (1*\xx,0*\yy) {\sage{red}{2}};
\node (v3) at (1*\xx,8*\yy) {\sage{red}{3}};
\node (v4) at (2*\xx,-10*\yy) {\sage{cyan}{4}};
\node (v5) at (2*\xx,-6*\yy) {\sage{yellow}{5}};
\node (v6) at (2*\xx,-2*\yy) {\sage{yellow}{6}};
\node (v7) at (2*\xx,2*\yy) {\sage{yellow}{7}};
\node (v8) at (2*\xx,6*\yy) {\sage{cyan}{8}};
\node (v9) at (2*\xx,10*\yy) {\sage{cyan}{9}};
\node (v10) at (3*\xx,-11*\yy) {\sage{cyan}{10}};
\node (v11) at (3*\xx,-9*\yy) {\sage{green}{11}};
\node (v12) at (3*\xx,-7*\yy) {\sage{magenta}{12}};
\node (v13) at (3*\xx,-5*\yy) {\sage{magenta}{13}};
\node (v14) at (3*\xx,-3*\yy) {\sage{magenta}{14}};
\node (v15) at (3*\xx,-1*\yy) {\sage{green}{15}};
\node (v16) at (3*\xx,1*\yy) {\sage{magenta}{16}};
\node (v17) at (3*\xx,3*\yy) {\sage{gray}{17}};
\node (v18) at (3*\xx,5*\yy) {\sage{magenta}{18}};
\node (v19) at (3*\xx,7*\yy) {\sage{green}{19}};
\node (v20) at (3*\xx,9*\yy) {\sage{magenta}{20}};
\node (v21) at (3*\xx,11*\yy) {\sage{gray}{21}};
\draw[->] (v0) -- node [below, sloped] {\footnotesize{G = neutro. }} (v1);
\draw[->] (v0) -- node [above, sloped] {\footnotesize{G = conv. }} (v2);
\draw[->] (v0) -- node [above, sloped] {\footnotesize{G = non-conv. }} (v3);
\draw[->] (v1) --  node [below, sloped] {\footnotesize{F = bronco.}} (v5);
\draw[->] (v1) --  node [above, sloped] {\footnotesize{F = angio.}} (v6);
\draw[->] (v2) --  node [below, sloped] {\footnotesize{F = bronco.}} (v7);
\draw[->] (v2) --  node [above, sloped] {\footnotesize{F = angio.}} (v8);
\draw[->] (v3) --  node [below, sloped] {\footnotesize{F = bronco.}} (v9);
\draw[->] (v3) --  node [above, sloped] {\footnotesize{F = angio.}} (v10);
\end{tikzpicture}
}
\caption{Staged tree learned using the hill-climbing algorithm (left) and the CSBHC algorithm (right) over the aspects of everyday life data with variables' order S, F, G, B, L.\label{fig:lifehc}}
\end{figure}

==> images/bn1.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}
\renewcommand{\xx}{3}
\renewcommand{\yy}{1.5}
\node (U) at (0*\xx,0*\yy){\stages{white}{U}};
\node (G) at (1*\xx,0*\yy){\stages{white}{G}};
\node (I) at (0*\xx,1*\yy){\stages{white}{I}};
\node (F) at (1*\xx,1*\yy){\stages{white}{F}};
\node (D) at (0.5*\xx,2*\yy){\stages{white}{D}};
\draw[->,black, line width = 1.3pt] (U) -- (I);
\draw[->,black, line width = 1.3pt] (G) -- (F);
\draw[->,black, line width = 1.3pt] (F) -- (I);
\draw[->,black, line width = 1.3pt] (I) -- (D);
\end{tikzpicture}
\end{center}
\caption{BN for the aspects of everyday life data (left) as well as ALDAGs over the same data associated to the staged trees learned with BHC (center) and CSBHC  (right). The edge coloring is: red - context; blue - partial; violet - context/partial; green - local; black - total. \label{fig:life}}
\end{figure}

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> images/tree1.tex <==

\begin{figure*}
\centering
\scalebox{0.5}{
\begin{tikzpicture}
\renewcommand{\xx}{4}
\renewcommand{\yy}{1.6}
\node (v0) at (0*\xx,0*\yy) {\sage{white}{0}};
\node (v1) at (1*\xx,-8*\yy) {\sage{pink}{1}};
\node (v2) at (1*\xx,0*\yy) {\sage{red}{2}};
\node (v3) at (1*\xx,8*\yy) {\sage{red}{3}};
\node (v4) at (2*\xx,-10*\yy) {\sage{cyan}{4}};
\node (v5) at (2*\xx,-6*\yy) {\sage{yellow}{5}};
\node (v6) at (2*\xx,-2*\yy) {\sage{yellow}{6}};
\node (v7) at (2*\xx,2*\yy) {\sage{yellow}{7}};
\node (v8) at (2*\xx,6*\yy) {\sage{cyan}{8}};
\node (v9) at (2*\xx,10*\yy) {\sage{cyan}{9}};
\node (v10) at (3*\xx,-11*\yy) {\leaf};
\node (v11) at (3*\xx,-9*\yy) {\sage{green}{10}};
\node (v12) at (3*\xx,-7*\yy) {\sage{teal}{16}};
\node (v13) at (3*\xx,-5*\yy) {\sage{magenta}{11}};
\node (v14) at (3*\xx,-3*\yy) {\sage{lime}{17}};
\node (v15) at (3*\xx,-1*\yy) {\sage{green}{12}};
\node (v16) at (3*\xx,1*\yy) {\sage{violet}{18}};
\node (v17) at (3*\xx,3*\yy) {\sage{gray}{13}};
\node (v18) at (3*\xx,5*\yy) {\sage{lightgray}{19}};
\node (v19) at (3*\xx,7*\yy) {\sage{green}{14}};
\node (v20) at (3*\xx,9*\yy) {\sage{lightgray}{20}};
\node (v21) at (3*\xx,11*\yy) {\sage{gray}{15}};
\node (v24) at (4*\xx,-9.5*\yy) {\leaf};
\node (v25) at (4*\xx,-8.5*\yy) {\sage{orange}{21}};
\node (v26) at (4*\xx,-7.5*\yy) {\leaf};
\node (v27) at (4*\xx,-6.5*\yy) {\leaf};
\node (v28) at (4*\xx,-5.5*\yy) {\sage{orange}{22}};
\node (v29) at (4*\xx,-4.5*\yy) {\leaf};
\node (v30) at (4*\xx,-3.5*\yy) {\leaf};
\node (v31) at (4*\xx,-2.5*\yy) {\leaf};
\node (v32) at (4*\xx,-1.5*\yy) {\leaf};
\node (v33) at (4*\xx,-0.5*\yy) {\sage{violet}{23}};
\node (v34) at (4*\xx,0.5*\yy) {\leaf};
\node (v35) at (4*\xx,1.5*\yy) {\leaf};
\node (v36) at (4*\xx,2.5*\yy) {\sage{teal}{24}};
\node (v37) at (4*\xx,3.5*\yy) {\sage{olive}{25}};
\node (v38) at (4*\xx,4.5*\yy) {\leaf};
\node (v39) at (4*\xx,5.5*\yy) {\leaf};
\node (v40) at (4*\xx,6.5*\yy) {\leaf};
\node (v41) at (4*\xx,7.5*\yy) {\sage{lightgray}{26}};
\node (v42) at (4*\xx,8.5*\yy) {\leaf};
\node (v43) at (4*\xx,9.5*\yy) {\leaf};
\node (v44) at (4*\xx,10.5*\yy) {\sage{lime}{27}};
\node (v45) at (4*\xx,11.5*\yy) {\sage{olive}{28}};
\node (v52) at (5*\xx,-8.75*\yy) {\leaf};
\node (v53) at (5*\xx,-8.25*\yy) {\leaf};
\node (v58) at (5*\xx,-5.75*\yy) {\leaf};
\node (v59) at (5*\xx,-5.25*\yy) {\leaf};
\node (v68) at (5*\xx,-0.75*\yy) {\leaf};
\node (v69) at (5*\xx,-0.25*\yy) {\leaf};
\node (v74) at (5*\xx,2.25*\yy) {\leaf};
\node (v75) at (5*\xx,2.75*\yy) {\leaf};
\node (v76) at (5*\xx,3.25*\yy) {\leaf};
\node (v77) at (5*\xx,3.75*\yy) {\leaf};
\node (v84) at (5*\xx,7.25*\yy) {\leaf};
\node (v85) at (5*\xx,7.75*\yy) {\leaf};
\node (v90) at (5*\xx,10.25*\yy) {\leaf};
\node (v91) at (5*\xx,10.75*\yy) {\leaf};
\node (v92) at (5*\xx,11.25*\yy) {\leaf};
\node (v93) at (5*\xx,11.75*\yy) {\leaf};
\draw[->] (v0) -- node [below, sloped] {{G = neutro. (0.06) }} (v1);
\draw[->] (v0) -- node [above, sloped] {{G = conv. (0.72)}} (v2);
\draw[->] (v0) -- node [above, sloped] {{G = non-conv. (0.22)}} (v3);
\draw[->] (v1) --  node [below, sloped] {{F = bronco. (0.11)}} (v4);
\draw[->] (v1) --  node [above, sloped] {{F = angio. (0.89)}} (v5);
\draw[->] (v2) --  node [below, sloped] {{F = bronco. (0.58)}} (v6);
\draw[->] (v2) --  node [above, sloped] {{F = angio. (0.42)}} (v7);
\draw[->] (v3) --  node [below, sloped] {{F = bronco. (0.58)}} (v8);
\draw[->] (v3) --  node [above, sloped] {{F = angio. (0.42)}} (v9);
\draw[->] (v4) --  node [below, sloped] {{U = no (0.30)}} (v10);
\draw[->] (v4) --  node [above, sloped] {{U = yes (0.70)}} (v11);
\draw[->] (v5) --  node [below, sloped] {{U = no (0.57)}} (v12);
\draw[->] (v5) --  node [above, sloped] {{U = yes (0.43)}} (v13);
\draw[->] (v6) --  node [below, sloped] {{U = no (0.57)}} (v14);
\draw[->] (v6) --  node [above, sloped] {{U = yes (0.43)}} (v15);
\draw[->] (v7) --  node [below, sloped] {{U = no (0.57)}} (v16);
\draw[->] (v7) --  node [above, sloped] {{U = yes (0.43)}} (v17);
\draw[->] (v8) --  node [below, sloped] {{U = no (0.30)}} (v18);
\draw[->] (v8) --  node [above, sloped] {{U = yes (0.70)}} (v19);
\draw[->] (v9) --  node [below, sloped] {{U = no (0.30)}} (v20);
\draw[->] (v9) --  node [above, sloped] {{U = yes (0.70)}} (v21);
\draw[->] (v11) --  node [below, sloped] {{I = no (0.00)}} (v24);
\draw[->] (v11) --  node [above, sloped] {{I = yes (1.00)}} (v25);
\draw[->] (v12) --  node [below, sloped] {{D = no (0.73)}} (v26);
\draw[->] (v12) --  node [above, sloped] {{D = yes (0.27)}} (v27);
\draw[->] (v13) --  node [below, sloped] {{I = no (1.00)}} (v28);
\draw[->] (v13) --  node [above, sloped] {{I = yes (0.00)}} (v29);
\draw[->] (v14) --  node [below, sloped] {{D = no (0.82)}} (v30);
\draw[->] (v14) --  node [above, sloped] {{D = yes (0.18)}} (v31);
\draw[->] (v15) --  node [below, sloped] {{I = no (0.00)}} (v32);
\draw[->] (v15) --  node [above, sloped] {{I = yes (1.00)}} (v33);
\draw[->] (v16) --  node [below, sloped] {{D = no (0.67)}} (v34);
\draw[->] (v16) --  node [above, sloped] {{D = yes (0.33)}} (v35);
\draw[->] (v17) --  node [below, sloped] {{I = no (0.16)}} (v36);
\draw[->] (v17) --  node [above, sloped] {{I = yes (0.84)}} (v37);
\draw[->] (v18) --  node [below, sloped] {{D = no (0.50)}} (v38);
\draw[->] (v18) --  node [above, sloped] {{D = yes (0.50)}} (v39);
\draw[->] (v19) --  node [below, sloped] {{I = no (0.00)}} (v40);
\draw[->] (v19) --  node [above, sloped] {{I = yes (1.00)}} (v41);
\draw[->] (v20) --  node [below, sloped] {{D = no (0.50)}} (v42);
\draw[->] (v20) --  node [above, sloped] {{D = yes (0.50)}} (v43);
\draw[->] (v21) --  node [below, sloped] {{I = no (0.16)}} (v44);
\draw[->] (v21) --  node [above, sloped] {{I = yes (0.84)}} (v45);
\draw[->] (v25) --  node [below, sloped] {{D = no (0.00)}} (v52);
\draw[->] (v25) --  node [above, sloped] {{D = yes (1.00)}} (v53);
\draw[->] (v28) --  node [below, sloped] {{D = no (0.00)}} (v58);
\draw[->] (v28) --  node [above, sloped] {{D = yes (1.00)}} (v59);
\draw[->] (v33) --  node [below, sloped] {{D = no (0.67)}} (v68);
\draw[->] (v33) --  node [above, sloped] {{D = yes (0.33)}} (v69);
\draw[->] (v36) --  node [below, sloped] {{D = no (0.73)}} (v74);
\draw[->] (v36) --  node [above, sloped] {{D = yes (0.23)}} (v75);
\draw[->] (v37) --  node [below, sloped] {{D = no (0.41)}} (v76);
\draw[->] (v37) --  node [above, sloped] {{D = yes (0.59)}} (v77);
\draw[->] (v41) --  node [below, sloped] {{D = no (0.50)}} (v84);
\draw[->] (v41) --  node [above, sloped] {{D = yes (0.50)}} (v85);
\draw[->] (v44) --  node [below, sloped] {{D = no (0.82)}} (v90);
\draw[->] (v44) --  node [above, sloped] {{D = yes (0.18)}} (v91);
\draw[->] (v45) --  node [below, sloped] {{D = no (0.41)}} (v92);
\draw[->] (v45) --  node [above, sloped] {{D = yes (0.59)}} (v93);
\end{tikzpicture}
}
\caption{Staged tree over the variables GROUP, ANGIOINVASIVE PATTERN, ICU, INTUBUTATION, and DEATH.\label{fig:lifehc}}
\end{figure*}

==> images/tree2.tex <==

\begin{figure*}
\centering
\scalebox{0.5}{
\begin{tikzpicture}
\renewcommand{\xx}{4}
\renewcommand{\yy}{1.6}
\node (v0) at (0*\xx,0*\yy) {\sage{white}{0}};
\node (v1) at (1*\xx,-8*\yy) {\sage{pink}{1}};
\node (v2) at (1*\xx,0*\yy) {\sage{red}{2}};
\node (v3) at (1*\xx,8*\yy) {\sage{red}{3}};
\node (v4) at (2*\xx,-10*\yy) {\sage{cyan}{4}};
\node (v5) at (2*\xx,-6*\yy) {\sage{yellow}{5}};
\node (v6) at (2*\xx,-2*\yy) {\sage{yellow}{6}};
\node (v7) at (2*\xx,2*\yy) {\sage{yellow}{7}};
\node (v8) at (2*\xx,6*\yy) {\sage{cyan}{8}};
\node (v9) at (2*\xx,10*\yy) {\sage{cyan}{9}};
\node (v10) at (3*\xx,-11*\yy) {\leaf};
\node (v11) at (3*\xx,-9*\yy) {\sage{green}{10}};
\node (v12) at (3*\xx,-7*\yy) {\sage{teal}{16}};
\node (v13) at (3*\xx,-5*\yy) {\sage{magenta}{11}};
\node (v14) at (3*\xx,-3*\yy) {\sage{lime}{17}};
\node (v15) at (3*\xx,-1*\yy) {\sage{green}{12}};
\node (v16) at (3*\xx,1*\yy) {\sage{teal}{18}};
\node (v17) at (3*\xx,3*\yy) {\sage{gray}{13}};
\node (v18) at (3*\xx,5*\yy) {\sage{violet}{19}};
\node (v19) at (3*\xx,7*\yy) {\sage{green}{14}};
\node (v20) at (3*\xx,9*\yy) {\sage{violet}{20}};
\node (v21) at (3*\xx,11*\yy) {\sage{gray}{15}};
\node (v24) at (4*\xx,-9.5*\yy) {\leaf};
\node (v25) at (4*\xx,-8.5*\yy) {\sage{orange}{21}};
\node (v26) at (4*\xx,-7.5*\yy) {\leaf};
\node (v27) at (4*\xx,-6.5*\yy) {\leaf};
\node (v28) at (4*\xx,-5.5*\yy) {\sage{orange}{22}};
\node (v29) at (4*\xx,-4.5*\yy) {\leaf};
\node (v30) at (4*\xx,-3.5*\yy) {\leaf};
\node (v31) at (4*\xx,-2.5*\yy) {\leaf};
\node (v32) at (4*\xx,-1.5*\yy) {\leaf};
\node (v33) at (4*\xx,-0.5*\yy) {\sage{violet}{23}};
\node (v34) at (4*\xx,0.5*\yy) {\leaf};
\node (v35) at (4*\xx,1.5*\yy) {\leaf};
\node (v36) at (4*\xx,2.5*\yy) {\sage{violet}{24}};
\node (v37) at (4*\xx,3.5*\yy) {\sage{olive}{25}};
\node (v38) at (4*\xx,4.5*\yy) {\leaf};
\node (v39) at (4*\xx,5.5*\yy) {\leaf};
\node (v40) at (4*\xx,6.5*\yy) {\leaf};
\node (v41) at (4*\xx,7.5*\yy) {\sage{violet}{26}};
\node (v42) at (4*\xx,8.5*\yy) {\leaf};
\node (v43) at (4*\xx,9.5*\yy) {\leaf};
\node (v44) at (4*\xx,10.5*\yy) {\sage{lime}{27}};
\node (v45) at (4*\xx,11.5*\yy) {\sage{olive}{28}};
\node (v52) at (5*\xx,-8.75*\yy) {\leaf};
\node (v53) at (5*\xx,-8.25*\yy) {\leaf};
\node (v58) at (5*\xx,-5.75*\yy) {\leaf};
\node (v59) at (5*\xx,-5.25*\yy) {\leaf};
\node (v68) at (5*\xx,-0.75*\yy) {\leaf};
\node (v69) at (5*\xx,-0.25*\yy) {\leaf};
\node (v74) at (5*\xx,2*\yy) {\leaf};
\node (v75) at (5*\xx,2.5*\yy) {\leaf};
\node (v76) at (5*\xx,3.25*\yy) {\leaf};
\node (v77) at (5*\xx,3.75*\yy) {\leaf};
\node (v84) at (5*\xx,7*\yy) {\leaf};
\node (v85) at (5*\xx,7.5*\yy) {\leaf};
\node (v90) at (5*\xx,10*\yy) {\leaf};
\node (v91) at (5*\xx,10.5*\yy) {\leaf};
\node (v92) at (5*\xx,11.25*\yy) {\leaf};
\node (v93) at (5*\xx,11.75*\yy) {\leaf};
\draw[->] (v0) -- node [below, sloped] {{\large{G = neutro. (0.06) }}} (v1);
\draw[->] (v0) -- node [above, sloped] {{\large{G = conv. (0.72)}}} (v2);
\draw[->] (v0) -- node [above, sloped] {{\large{G = no-conv. (0.22)}} }(v3);
\draw[->] (v1) --  node [below, sloped] {{\large{P = bronco. (0.11)}}} (v4);
\draw[->] (v1) --  node [above, sloped] {{\large{P = angio. (0.89)}}} (v5);
\draw[->] (v2) --  node [below, sloped] {{\large{P = bronco. (0.58)}} }(v6);
\draw[->] (v2) --  node [above, sloped] {{\large{P = angio. (0.42)}} }(v7);
\draw[->] (v3) --  node [below, sloped] {{\large{P = bronco. (0.58)}}} (v8);
\draw[->] (v3) --  node [above, sloped] {{\large{P = angio. (0.42)}}} (v9);
\draw[->] (v4) --  node [below, sloped] {{\large{U = no (0.30)}}} (v10);
\draw[->] (v4) --  node [above, sloped] {{\large{U = si (0.70)}}} (v11);
\draw[->] (v5) --  node [below, sloped] {{\large{U = no (0.57)}}} (v12);
\draw[->] (v5) --  node [above, sloped] {{\large{U = si (0.43)}}} (v13);
\draw[->] (v6) --  node [below, sloped] {{\large{U = no (0.57)}}} (v14);
\draw[->] (v6) --  node [above, sloped] {{\large{U = si (0.43)}}} (v15);
\draw[->] (v7) --  node [below, sloped] {{\large{U = no (0.57)}}} (v16);
\draw[->] (v7) --  node [above, sloped] {{\large{U = si (0.43)}}} (v17);
\draw[->] (v8) --  node [below, sloped] {{\large{U = no (0.30)}}} (v18);
\draw[->] (v8) --  node [above, sloped] {{\large{U = si (0.70)}}} (v19);
\draw[->] (v9) --  node [below, sloped] {{\large{U = no (0.30)}}} (v20);
\draw[->] (v9) --  node [above, sloped] {{\large{U = si (0.70)}} }(v21);
\draw[->] (v11) --  node [below, sloped] {{\large{I = no (0.00)}}} (v24);
\draw[->] (v11) --  node [above, sloped] {{\large{I = si (1.00)}}} (v25);
\draw[->] (v12) --  node [below, sloped] {{\large{M = no (0.71)}}} (v26);
\draw[->] (v12) --  node [above, sloped] {{\large{M = si (0.29)}}} (v27);
\draw[->] (v13) --  node [below, sloped] {{\large{I = no (1.00)}}} (v28);
\draw[->] (v13) --  node [above, sloped] {{\large{I = si (0.00)}}} (v29);
\draw[->] (v14) --  node [below, sloped] {{\large{M = no (0.82)}}} (v30);
\draw[->] (v14) --  node [above, sloped] {{\large{M = si (0.18)}}} (v31);
\draw[->] (v15) --  node [below, sloped] {{\large{I = no (0.00)}}} (v32);
\draw[->] (v15) --  node [above, sloped] {{\large{I = si (1.00)}}} (v33);
\draw[->] (v16) --  node [below, sloped] {{\large{M = no (0.71)}}} (v34);
\draw[->] (v16) --  node [above, sloped] {{\large{M = si (0.29)}}} (v35);
\draw[->] (v17) --  node [below, sloped] {{\large{I = no (0.16)}}} (v36);
\draw[->] (v17) --  node [above, sloped] {{\large{I = si (0.84)}}} (v37);
\draw[->] (v18) --  node [below, sloped] {{\large{M = no (0.56)}}} (v38);
\draw[->] (v18) --  node [above, sloped] {{\large{M = si (0.44)}}} (v39);
\draw[->] (v19) --  node [below, sloped] {{\large{I = no (0.00)}}} (v40);
\draw[->] (v19) --  node [above, sloped] {{\large{I = si (1.00)}}} (v41);
\draw[->] (v20) --  node [below, sloped] {{\large{M = no (0.56)}}} (v42);
\draw[->] (v20) --  node [above, sloped] {{\large{M = si (0.44)}}} (v43);
\draw[->] (v21) --  node [below, sloped] {{\large{I = no (0.16)}}} (v44);
\draw[->] (v21) --  node [above, sloped] {{\large{I = si (0.84)}}} (v45);
\draw[->] (v25) --  node [below, sloped] {{\large{M = no (0.00)}}} (v52);
\draw[->] (v25) --  node [above, sloped] {{\large{M = si (1.00)}}} (v53);
\draw[->] (v28) --  node [below, sloped] {{\large{M = no (0.00)}}} (v58);
\draw[->] (v28) --  node [above, sloped] {{\large{M = si (1.00)}}} (v59);
\draw[->] (v33) --  node [below, sloped] {{\large{M = no (0.56)}}} (v68);
\draw[->] (v33) --  node [above, sloped] {{\large{M = si (0.44)}}} (v69);
\draw[->] (v36) --  node [below, sloped] {{\large{M = no (0.56)}}} (v74);
\draw[->] (v36) --  node [above, sloped] {{\large{M = si (0.44)}}} (v75);
\draw[->] (v37) --  node [below, sloped] {{\large{M = no (0.37)}}} (v76);
\draw[->] (v37) --  node [above, sloped] {{\large{M = si (0.63)}}} (v77);
\draw[->] (v41) --  node [below, sloped] {{\large{M = no (0.56)}}} (v84);
\draw[->] (v41) --  node [above, sloped] {{\large{M = si (0.44)}}} (v85);
\draw[->] (v44) --  node [below, sloped] {{\large{M = no (0.82)}}} (v90);
\draw[->] (v44) --  node [above, sloped] {{\large{M = si (0.18)}}} (v91);
\draw[->] (v45) --  node [below, sloped] {{\large{M = no (0.37)}}} (v92);
\draw[->] (v45) --  node [above, sloped] {{\large{M = si (0.63)}}} (v93);
\end{tikzpicture}
}
\caption{Staged tree over the variables GROUP, ANGIOINVASIVE PATTERN, ICU, INTUBUTATION, and DEATH.\label{fig:lifehc}}
\end{figure*}

==> tables/MI.tex <==
\begin{sidewaystable}
\floatconts
  {table:mi}%
  {\caption{Variables considered for the population under study, acronyms and variables' levels.}}%
  {%
  \scalebox{0.7}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
\hline
&Marginal & GROUP & IS & FORM &  ICU &  CMV &   DESN &  TUMOR & NEUTRO & CS   & IOE    \\
\hline
GROUP &   0.0060 &  &0.0036($-38$\%) & 0.0058($-0.7$\%) & 0.0085($+47$\%) & 0.0051($-11$\%)& 0.0059($+2.0$\%)& 0.0059($+1.8$\%) & 0.0049($-16$\%) & 0.0040($-31$\%) &0.0052($-11$\%)\\
\hline
IS   &   0.0022  & 0.0000($-99$\%)  & & 0.0022($+1.4$\%) & 0.0020($-10$\%) & 0.0016($-26$\%)& 0.0023($+3.1$\%)& 0.0021($-4.8$\%) & 0.0024($+9.8$\%)&0.0010($-55$\%) & 0.0019($-14$\%)\\
\hline
FORM &   0.0000  & 0.0000($-56$\%) &0.0001($+44$\%) & &0.0000($-98$\%)&0.0001($+9.2$\%)& 0.0008($+958$\%) &  0.0003($+313$\%)& 0.0002($+229$\%) & 0.0000($-86$\%)& 0.0001($-15$\%)\\
\hline
ICU &    0.0160  & 0.0187($+17$\%) &0.0158($+1.4$\%) &0.0159($-0.4$\%)  & & 0.0155($-3.2$\%)& 0.0157($-2.2$\%) & 0.0153($-4.5$\%) &0.0173($+8.3$\%) & 0.0136($-15$\%) &0.0156($-2.5$\%)\\
\hline
CMV &     0.0008 &0.0001($-85$\%) &0.0002($-72$\%) & 0.0008($+0.8$\%)     & 0.0003($-64$\%) & & 0.0008($-0.5$\%) &0.0008($-3.4$\%) &0.0007($-16$\%) &  0.0008($+2.2$\%)& 0.0007($-12$\%)\\
\hline
DESN &   0.0004 & 0.0005($+33$\%) &0.0004($+19$\%) & 0.0011($+197$\%)& 0.0000($-100\%$)&0.0004($-1.1$\%)& 
 & 0.0003($-8.2$\%)&0.0003($-2.7$\%) & 0.0004($+17$\%) & 0.0004($+3.2$\%)\\
\hline
TUMOR &   0.0007  &   
 0.0008($+14$\%) &0.0006($-15$\%) & 0.0010($+31$\%) & 0.0000($-100$\%) & 0.0007($-3.8$\%)& 0.0007($-4.0$\%) & & 0.0009($+25$\%)  &  0.0005($-30$\%) &0.0007($-5.8$\%)\\
\hline
NEUTRO &  0.0009 & 0.0000($-100$\%)  &0.0011($+24$\%) & 0.0011($+18$\%) & 0.0022($+145$\%) & 0.0008($-14$\%)& 0.0009($-1.0$\%) & 0.0011($+20$\%)& &0.0013($+43$\%)& 0.0010($+4.1$\%)\\
\hline
CS &    0.0029  & 0.0011($-61$\%) &0.0017($-42$\%) & 0.0029($-2.1$\%)  & 0.0005($-84$\%) &0.0029($+0.6$\%) & 0.0030($+2.0$\%) &0.0027($-7.5$\%) &0.0033($+13$\%) &  & 0.0024($-17$\%)\\
\hline
IOE &     0.0006 & 0.0000($-100$\%) &0.0003($-50$\%) & 0.0006($-1.7$\%) & 0.0002($-62$\%)& 0.0005($-15$\%)& 0.0007($+1.7$\%)&  0.0006($-6.5$\%)& 0.0007($+5.9$\%) & 0.0001($-78$\%) & \\
\hline
\end{tabular}}}
\end{sidewaystable}

==> tables/MI2.tex <==
\begin{table*}
\floatconts
  {table:mi}%
  {\caption{Variables considered for the population under study, acronyms and variables' levels.}}%
  {%
  \scalebox{0.8}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
& \textbf{Marginal} & \textbf{GR} & \textbf{IM} & \textbf{AP} &  \textbf{ICU} &  \textbf{CMV}   \\
\hline
\textbf{GR} &   0.0060 &  &0.0036($-38$\%) & 0.0058($-0.7$\%) & 0.0085($+47$\%) & 0.0051($-11$\%)\\
\hline
\textbf{IM}   &   0.0022  & 0.0000($-99$\%)  & & 0.0022($+1.4$\%) & 0.0020($-10$\%) & 0.0016($-26$\%)\\
\hline
\textbf{AP} &   0.0000  & 0.0000($-56$\%) &0.0001($+44$\%) & &0.0000($-98$\%)&0.0001($+9.2$\%)\\
\hline
\textbf{ICU} &    0.0160  & 0.0187($+17$\%) &0.0158($+1.4$\%) &0.0159($-0.4$\%)  & & 0.0155($-3.2$\%)\\
\hline
\textbf{CMV} &     0.0008 &0.0001($-85$\%) &0.0002($-72$\%) & 0.0008($+0.8$\%)     & 0.0003($-64$\%) & \\
\hline
\textbf{MN} &   0.0004 & 0.0005($+33$\%) &0.0004($+19$\%) & 0.0011($+197$\%)& 0.0000($-100\%$)&0.0004($-1.1$\%)\\
\hline
\textbf{UST} &   0.0007  &   
 0.0008($+14$\%) &0.0006($-15$\%) & 0.0010($+31$\%) & 0.0000($-100$\%) & 0.0007($-3.8$\%)\\
\hline
\textbf{PN} &  0.0009 & 0.0000($-100$\%)  &0.0011($+24$\%) & 0.0011($+18$\%) & 0.0022($+145$\%) & 0.0008($-14$\%)\\
\hline
\textbf{SC} &    0.0029  & 0.0011($-61$\%) &0.0017($-42$\%) & 0.0029($-2.1$\%)  & 0.0005($-84$\%) &0.0029($+0.6$\%) \\
\hline
\textbf{VP} &     0.0006 & 0.0000($-100$\%) &0.0003($-50$\%) & 0.0006($-1.7$\%) & 0.0002($-62$\%)& 0.0005($-15$\%)\\
\hline
\\
\hline 
& \textbf{Marginal} &  \textbf{MN}&  \textbf{UST} & \textbf{PN} & \textbf{SC}   & \textbf{VP}  \\
\hline
\textbf{GR} &  0.0060& 0.0059($+2.0$\%)& 0.0059($+1.8$\%) & 0.0049($-16$\%) & 0.0040($-31$\%) &0.0052($-11$\%)  \\
\hline
\textbf{IM} &     0.0022 & 0.0023($+3.1$\%)& 0.0021($-4.8$\%) & 0.0024($+9.8$\%)&0.0010($-55$\%) & 0.0019($-14$\%)  \\
\hline
\textbf{AP} &   0.0000  & 0.0008($+958$\%) &  0.0003($+313$\%)& 0.0002($+229$\%) & 0.0000($-86$\%)& 0.0001($-15$\%)   \\
\hline
\textbf{ICU} &     0.0160 & 0.0157($-2.2$\%) & 0.0153($-4.5$\%) &0.0173($+8.3$\%) & 0.0136($-15$\%) &0.0156($-2.5$\%)       \\
\hline
\textbf{CMV} &     0.0008 & 0.0008($-0.5$\%) &0.0008($-3.4$\%) &0.0007($-16$\%) &  0.0008($+2.2$\%)& 0.0007($-12$\%)    \\
\hline
\textbf{MN} &     0.0004 & 
 & 0.0003($-8.2$\%)&0.0003($-2.7$\%) & 0.0004($+17$\%) & 0.0004($+3.2$\%)    \\
\hline
\textbf{UST} &   0.0007  & 0.0007($-4.0$\%) & & 0.0009($+25$\%)  &  0.0005($-30$\%) &0.0007($-5.8$\%)  \\
\hline
\textbf{PN} &   0.0009  & 0.0009($-1.0$\%) & 0.0011($+20$\%)& &0.0013($+43$\%)& 0.0010($+4.1$\%)    \\
\hline
\textbf{SC} &     0.0029 & 0.0030($+2.0$\%) &0.0027($-7.5$\%) &0.0033($+13$\%) &  & 0.0024($-17$\%)        \\
\hline
\textbf{VP} &     0.0006  & 0.0007($+1.7$\%)&  0.0006($-6.5$\%)& 0.0007($+5.9$\%) & 0.0001($-78$\%) &      \\
\hline
\end{tabular}}}
\end{table*}

==> tables/logistic.tex <==
\begin{table*}
\floatconts
  {table:logistic}%
  {\caption{Odds ratios, confidence intervals and p-values for univariate logistic regressions to predict death.}}%
  {
  \scalebox{0.8}{
  \renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Response & Predictor & Term & OR & CI.Low & CI.High & P-value\\
\hline
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Neutropenic (Intercept)} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{3.02} & \cellcolor{gray!6}{0.74}\\
\hline
\textbf{DEATH}&\textbf{GROUP} & Conventional & 0.71 & 0.18 & 3.01 & 0.62\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Non-Conventional} & \cellcolor{gray!6}{1.10} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{5.18} & \cellcolor{gray!6}{0.90}\\
\hline
\textbf{DEATH}&\textbf{RADIOLOGICAL PATTERN} & Bronco. (Intercept) & 0.51 & 0.32 & 0.80 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{RADIOLOGICAL PATTERN}} & \cellcolor{gray!6}{Angio.} & \cellcolor{gray!6}{1.64} & \cellcolor{gray!6}{0.84} & \cellcolor{gray!6}{3.22} & \cellcolor{gray!6}{0.15}\\
\hline
\textbf{DEATH}&\textbf{ICU} & No (Intercept) & 0.37 & 0.22 & 0.61 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{ICU}} & \cellcolor{gray!6}{Yes} & \cellcolor{gray!6}{2.85} & \cellcolor{gray!6}{1.44} & \cellcolor{gray!6}{5.77} & \cellcolor{gray!6}{0.00}\\
\hline
\textbf{DEATH}&\textbf{INTUBATION} & No (Intercept) & 0.40 & 0.24 & 0.65 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{INTUBATION}} & \cellcolor{gray!6}{Yes} & \cellcolor{gray!6}{2.63} & \cellcolor{gray!6}{1.34} & \cellcolor{gray!6}{5.27} & \cellcolor{gray!6}{0.01}\\
\hline
\hline
\textbf{INTUBATION}&\textbf{GROUP} & Neutropenic (Intercept) & 0.13 & 0.01 & 0.68 & 0.05\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Conventional} & \cellcolor{gray!6}{5.77} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{109.0} & \cellcolor{gray!6}{0.10}\\
\hline
\textbf{INTUBATION}&\textbf{GROUP} & Non-Conventional & 15.2 & 2.37 & 302.8 & 0.02\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{RADIOLOGICAL PATTERN}} & \cellcolor{gray!6}{Bronco. (Intercept)} & \cellcolor{gray!6}{0.95} & \cellcolor{gray!6}{0.61} & \cellcolor{gray!6}{1.48} & \cellcolor{gray!6}{0.82}\\
\hline
\textbf{INTUBATION}&\textbf{RADIOLOGICAL PATTERN} & Angio. & 0.73 & 0.37 & 1.40 & 0.34\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{ICU}} & \cellcolor{gray!6}{No (Intercept)} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{Inf} & \cellcolor{gray!6}{0.99}\\
\hline
\textbf{INTUBATION}&\textbf{ICU} & Yes & 0.00 & 0.00 & Inf & 0.99\\
\hline
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Neutropenic (Intercept)} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{1.18} & \cellcolor{gray!6}{0.12}\\
\hline
\textbf{ICU}&\textbf{GROUP} & Conventional & 2.95 & 0.67 & 20.4 & 0.19\\
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Non-Conventional} & \cellcolor{gray!6}{7.70} & \cellcolor{gray!6}{1.54} & \cellcolor{gray!6}{58.3} & \cellcolor{gray!6}{0.02}\\
\hline
\textbf{ICU}&\textbf{RADIOLOGICAL PATTERN} & Bronco. (Intercept) & 0.95 & 0.61 & 1.48 & 0.82\\
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{RADIOLOGICAL PATTERN}} & \cellcolor{gray!6}{Angio.} & \cellcolor{gray!6}{1.05} & \cellcolor{gray!6}{0.55} & \cellcolor{gray!6}{2.02} & \cellcolor{gray!6}{0.88}\\
\hline
\end{tabular}}}
\end{table*}


==> tables/table_lasso.tex <==
\begin{table}[htbp]
\floatconts
  {table:lasso}%
  {\caption{Estimated ORs for LASSO logistic regression with 2-way interactions to predict DEATH.}}%
  {
  \scalebox{0.6}{
\begin{tabular}{c|c}
\hline
Term & OR\\
\hline
\textbf{\cellcolor{gray!6}{Intercept}} & \cellcolor{gray!6}{0.45}\\
\hline
\textbf{GROUP = conventional} & 0.78\\
\hline
\textbf{\cellcolor{gray!6}{GROUP = non-conventional}} & \cellcolor{gray!6}{1.17}\\
\hline
\textbf{FORM = angioinvasive} & 1.30\\
\hline
\textbf{\cellcolor{gray!6}{ICU = yes}} & \cellcolor{gray!6}{1.00}\\
\hline
\textbf{INTUBATION = yes} & 1.68\\
\hline
\textbf{\cellcolor{gray!6}{GROUP = conventional \& FORM = angioinvasive}} & \cellcolor{gray!6}{1.00}\\
\hline
\textbf{GROUP = non-conventional \& FORM = angioinvasive} & 1.00\\
\hline
\textbf{\cellcolor{gray!6}{GROUP = conventional \& ICU = yes}} & \cellcolor{gray!6}{1.00}\\
\hline
\textbf{GROUP = non-conventional \& ICU = yes} & 1.00\\
\hline
\textbf{\cellcolor{gray!6}{GROUP = conventional \& INTUBATION = yes}} & \cellcolor{gray!6}{1.00}\\
\hline
\textbf{GROUP = non-conventional \& INTUBATION = yes} & 1.00\\
\hline
\textbf{\cellcolor{gray!6}{FORM = angioinvasive \& ICU = yes}} & \cellcolor{gray!6}{1.00}\\
\hline
\textbf{FORM = angioinvasive \& INTUBATION = yes} & 1.37\\
\hline
\textbf{\cellcolor{gray!6}{ICU = yes \& INTUBATION = yes}} & \cellcolor{gray!6}{1.00}\\
\hline
\end{tabular}}}
\end{table}


==> tables/table_logistic.tex <==
\begin{table}[htbp]
\floatconts
  {table:logistic}%
  {\caption{Odds ratios, confidence intervals and p-values for univariate logistic regressions to predict death.}}%
  {
  \scalebox{0.5}{
\begin{tabular}[t]{>{\centering\arraybackslash}p{3cm}|c|c|c|c|c|c}
\hline
Response & Predictor & Term & OR & CI.Low & CI.High & P-value\\
\hline
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Neutropenic (Intercept)} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{3.02} & \cellcolor{gray!6}{0.74}\\
\hline
\textbf{DEATH}&\textbf{GROUP} & Conventional & 0.71 & 0.18 & 3.01 & 0.62\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Non-Conventional} & \cellcolor{gray!6}{1.10} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{5.18} & \cellcolor{gray!6}{0.90}\\
\hline
\textbf{DEATH}&\textbf{RADIOLOGICAL PATTERN} & Bronco (Intercept) & 0.48 & 0.30 & 0.76 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{ANGIOINVASIVE PATTERN}} & \cellcolor{gray!6}{Si} & \cellcolor{gray!6}{1.63} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{3.21} & \cellcolor{gray!6}{0.16}\\
\hline
\textbf{DEATH}&\textbf{ICU} & No (Intercept) & 0.40 & 0.23 & 0.65 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{ICU}} & \cellcolor{gray!6}{Yes} & \cellcolor{gray!6}{2.26} & \cellcolor{gray!6}{1.15} & \cellcolor{gray!6}{4.53} & \cellcolor{gray!6}{0.02}\\
\hline
\textbf{DEATH}&\textbf{INTUBATION} & No (Intercept) & 0.40 & 0.24 & 0.65 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{DEATH}}&\textbf{\cellcolor{gray!6}{INTUBATION}} & \cellcolor{gray!6}{Yes} & \cellcolor{gray!6}{2.33} & \cellcolor{gray!6}{1.18} & \cellcolor{gray!6}{4.67} & \cellcolor{gray!6}{0.02}\\
\hline
\hline
\textbf{INTUBATION}&\textbf{GROUP} & Neutropenic (Intercept) & 0.13 & 0.01 & 0.68 & 0.05\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Conventional} & \cellcolor{gray!6}{5.77} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{109.0} & \cellcolor{gray!6}{0.10}\\
\hline
\textbf{INTUBATION}&\textbf{GROUP} & Non-Conventional & 15.2 & 2.37 & 302.8 & 0.02\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{FORM}} & \cellcolor{gray!6}{Bronocinvasive (Intercept)} & \cellcolor{gray!6}{0.95} & \cellcolor{gray!6}{0.61} & \cellcolor{gray!6}{1.48} & \cellcolor{gray!6}{0.82}\\
\hline
\textbf{INTUBATION}&\textbf{FORM} & Angioinvasive & 0.73 & 0.37 & 1.40 & 0.34\\
\hline
\textbf{\cellcolor{gray!6}{INTUBATION}}&\textbf{\cellcolor{gray!6}{ICU}} & \cellcolor{gray!6}{No (Intercept)} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{Inf} & \cellcolor{gray!6}{0.99}\\
\hline
\textbf{INTUBATION}&\textbf{ICU} & Yes & 0.00 & 0.00 & Inf & 0.99\\
\hline
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Neutropenic (Intercept)} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{1.18} & \cellcolor{gray!6}{0.12}\\
\hline
\textbf{ICU}&\textbf{GROUP} & Conventional & 2.95 & 0.67 & 20.4 & 0.19\\
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{Non-Conventional} & \cellcolor{gray!6}{7.70} & \cellcolor{gray!6}{1.54} & \cellcolor{gray!6}{58.3} & \cellcolor{gray!6}{0.02}\\
\hline
\textbf{ICU}&\textbf{FORM} & Broncoinvasive (Intercept) & 0.48 & 0.30 & 0.76 & 0.00\\
\hline
\textbf{\cellcolor{gray!6}{ICU}}&\textbf{\cellcolor{gray!6}{FORM}} & \cellcolor{gray!6}{Angioinvasive} & \cellcolor{gray!6}{1.63} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{3.21} & \cellcolor{gray!6}{0.16}\\
\hline
\end{tabular}}}
\end{table}


==> tables/table_variables.tex <==
\begin{table*}
\floatconts
  {table:variables}%
  {\caption{Variables considered for the population under study, acronyms and variables' levels.}}%
  {%
  \scalebox{0.7}{
   \renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c}
\hline
Variable & Acronym & Levels\\
\hline
\textbf{\cellcolor{gray!6}{GROUP}} & \cellcolor{gray!6}{GR}& \cellcolor{gray!6}{Neutropenic/Conventional/Non-conventional}\\
\hline
\textbf{RADIOLOGICAL PATTERN} & RP & Angioinvasive/Broncoinvasive\\
\hline
\textbf{\cellcolor{gray!6}{ICU}} & \cellcolor{gray!6}{ICU}& \cellcolor{gray!6}{No/Yes}\\
\hline
\textbf{INTUBATION} & INT & No/Yes \\
\hline
\textbf{\cellcolor{gray!6}{DEATH}} & \cellcolor{gray!6}{D}& \cellcolor{gray!6}{No/Yes}\\
\hline
\textbf{IMMUNOTHERAPY} & IM & No/Yes \\
\hline
\textbf{\cellcolor{gray!6}{SYSTEMIC CORTICOIDS}} & \cellcolor{gray!6}{SC}& \cellcolor{gray!6}{No/Yes}\\
\hline
\textbf{PREVIOUS NEUTROPENIA} & PN & No/Yes\\
\hline
\textbf{\cellcolor{gray!6}{UNCONTROLLED SOLID TUMOR}} & \cellcolor{gray!6}{UST}& \cellcolor{gray!6}{No/Yes}\\
\hline
\textbf{MALNUTRITION} & MN& No/Yes\\
\hline
\textbf{\cellcolor{gray!6}{VIRAL PNEUMONIA}} & \cellcolor{gray!6}{VP}& \cellcolor{gray!6}{No/Yes}\\
\hline
\textbf{CMV INFECTION} & CMV & No/Yes\\
\hline
\end{tabular}}}
\end{table*}

==> tables/var.tex <==
\begin{table*}[htbp]
\floatconts
  {table:variables}%
  {\caption{Variables considered for the population under study, acronyms and variables' levels.}}%
  {%
  \scalebox{0.7}{
\begin{tabular}{lrr}
\toprule
Variable & Acronym & Levels\\
\midrule
\textbf{GROUP} & G& Neutropenic/Conventional/Non-conventional\\
\midrule
\textbf{FORM} & F & Angioinvasive/Broncoinvasive\\
\midrule
\textbf{ICU} & U& No/Yes\\
\midrule
\textbf{INTUBATION} & I & No/Yes \\
\midrule
\textbf{DEATH} & D& No/Yes\\
\midrule
\textbf{IMMUNOTHERAPY} & IM & No/Yes \\
\midrule
\textbf{SYSTEMIC CORTICOIDS} & SC& No/Yes\\
\midrule
\textbf{PREVIOUS NEUTROPENIA} & PN & No/Yes\\
\midrule
\textbf{UNCONTROLLED SOLID TUMOR} & UST& No/Yes\\
\midrule
\textbf{MALNUTRITION} & M& No/Yes\\
\midrule
\textbf{IRAL PNEUMONIA} & VP& No/Yes\\
\midrule
\textbf{COMMON CMV INFECTION} & CMV & No/Yes\\
\bottomrule
\end{tabular}}}
\end{table*}
